Agora: A Unified Asset Ecosystem Going Beyond Marketplaces and Cloud Services

Data, algorithms, and compute/storage infrastructure are key assets that drive data science and artificial intelligence applications. As providing all these assets requires a huge investment, data science and artificial intelligence technologies are currently dominated by a small number of providers who can afford these investments. This leads to lock-in effects and hinders features that require a flexible exchange of assets among users. In this vision paper, we present Agora, a unified asset ecosystem. The Agora system provides the technical infrastructure that allows for offering and using data and algorithms, as well as physical infrastructure components. Agora is designed as an open ecosystem of asset marketplaces and provides to a broad audience not only data but the entire data value chain (including computational resources and human expertise). Agora (i) leverages a fine-grained exchange of assets, (ii) allows for combining assets to novel applications, and (iii) flexibly executes such applications on available resources. As a result, Agora overcomes lock-in effects and removes entry barriers for new asset providers. In contrast to existing data management systems, Agora operates in a heavily decentralized and dynamic environment: Data, algorithms, and even compute resources are dynamically created, modified, and removed by different stakeholders. Agora presents novel research directions for the data management community as a whole: It requires to combine our traditional expertise in scalable data processing and management with infrastructure provisioning as well as economic and application aspects of data, algorithms, and infrastructure.

==> motivation.tex <==
We aim at designing an asset-centric ecosystem where everyone can offer and access all kinds of data-related assets and combine them to novel applications without any required expertise.
Assets cover the whole data science pipeline ranging from sensor data streams over machine learning models to specialized algorithms and from processing systems to compute and storage resources.
Such a fine-grained and easy exchange\steffen{text before does not talk about exchange and I would not use easy} of assets leads to three major benefits for the ecosystem community:\steffen{This is very confusing here, what will you describe, benefits, challenges, solutions, requirements? currently it is somehow a mixture of all and for what an ecosystem in general or for agora?}

\textbf{(1) Secondary use of existing assets.} We enable\steffen{to you mean we as an ecosystem or we as agora?} reuse of existing assets such as code reuse and data reuse:

\begin{example}[Secondary use of assets]\label{ex:secondary-usage}
A company that develops a navigation system records videos of test drives to improve their software.
The same data can be used for many other applications, such as planning of road maintenance and cataloging parking spots.
The data provider benefits from a financial reward and the data consumer gets\steffen{I think get} cheap access to high-quality data, which would not be available otherwise.
\end{example}


\noindent
Especially in Europe, small and medium-sized companies build the backbone of the economy.\steffen{again ref is missing}
These companies own a plethora of highly valuable assets.
However, because these assets are fragmented across companies, their economical potential remains unused as secondary asset usage is extremely rare.
A fine-grained asset sharing \steffen{would?} allows for combining existing resources to derive new insights and services.

\textbf{(2) Leveraging specializations.}
We\steffen{again who is we here?} leverage an ecosystem of highly specialized asset providers who focus on a particular set of assets and can provide their assets in very high quality.
Such an ecosystem is comparable with the automotive industry where many companies specialize in specific parts (e.g., brakes, tires, or lights), which get combined to one high-quality car.

\begin{example}[Specialized asset providers\steffen{mismatch between headline and this text}]\label{ex:secondary-usage}\steffen{label is wrong}
One company can specialize in operating a network of weather stations and providing accurate weather data in real-time.
Another company can develop a highly efficient stream join.
Yet another company combines both assets to correlate weather data with its \steffen{own?} sales data in order to predict revenues and estimate required logistics based on weather conditions. 
\end{example}

\noindent
Highly specialized providers can only operate economically if they can offer their assets through an open ecosystem without massive overhead.
We want to provide an easy way to offer, buy, and combine data, algorithms, software components and other data-related assets.
This \steffen{would?} allows small and medium-sized companies to offer data and software components that they would not be able to bring to market otherwise.
The ecosystem prevents the need for individual negotiations between providers and consumers, which allows for building applications combining assets from multiple vendors. 
Currently, many companies replicate the same fundamental software components and suffer from the non-availability of sufficiently large training data.
Our ecosystem aims to join forces to overcome these problems and to provide cheap and easy access to data science and AI\steffen{algos? technology?}.


\textbf{(3) Using equivalences.}
To optimize application execution, we \steffen{again who is we here?} make use of different physical implementations of the same logical operations, offered by different companies.
Available implementations have very different properties. They are using different programming languages (e.g., C++ or Java), tailored to different systems (e.g., Flink or Spark), optimized for specific hardware (CPU or GPU), and run highly parallelized or sequential \steffen{maybe add distributed here}.
In addition, each company can define different pricing for its algorithm.
Agora \steffen{now it is agora and not an ecosystem in general} can pick the best combination out of the available implementations based on the requirements of an application. 

\begin{example}[Using logical equivalence]\label{ex:secondary-usage}
A user has a fixed budget for sorting a large data set and wants to complete the task as fast as possible.
Several companies offer logically equivalent implementations of sorting algorithms.
Depending on the budget and the data characteristics, we\steffen{you mean the user or agora} can choose different algorithms:
If the budget is low, we will use a free algorithm that can run on some idling spot\steffen{???} instances.
If the budget is high, we will use a cluster of specialized nodes and run a more expensive algorithm, which supports GPU acceleration and high parallelism.
\end{example}

\noindent Our envisioned ecosystem provides access to a plethora of implementations one can use to improve performance and save cost.
The system should make it easy to replace implementations of particular operations or even do this automatically with respect to the optimization goals \steffen{maybe you mean requirements} of a user.

